Exact Convex Relaxation of Optimal Power Flow in Tree Networks

The optimal power flow (OPF) problem seeks to control power generation/demand to optimize certain objectives such as minimizing the generation cost or power loss in the network. It is becoming increasingly important for distribution networks, which are tree networks, due to the emergence of distributed generation and controllable loads. In this paper, we study the OPF problem in tree networks. The OPF problem is nonconvex. We prove that after a "small" modification to the OPF problem, its global optimum can be recovered via a second-order cone programming (SOCP) relaxation, under a "mild" condition that can be checked apriori. Empirical studies justify that the modification to OPF is "small" and that the "mild" condition holds for the IEEE 13-bus distribution network and two real-world networks with high penetration of distributed generation.

==> ExactRelaxation.tex <==

%%%%%%%%%%%%%%%%%%%%%
\section{Exact relaxation}
\label{sec: exact relaxation}
We provide sufficient conditions for exact SOCP relaxation in this section.
It motivates adding an additional constraint on power injections $(p,q)$ to OPF in Section \ref{sec: MOPF}. In Section \ref{sec: MOPF}, we show that not only the modified OPF problem has an exact
SOCP relaxation, but also its feasible set is close to that of the original OPF.
In Section \ref{sec: math}, we prove the sufficient conditions in detail.



Define the following functions of $p$ and $q$:
	\begin{eqnarray*}
	P_{ji}^\mathrm{lin}(p) \!\! & :=&\!\!  \sum_{k:j\in\hP_k} p_k, \qquad\qquad (i,j)\in\hL;  \label{lossless P}\\
	Q_{ji}^\mathrm{lin}(q) \!\! & :=&\!\!  \sum_{k:j\in\hP_k} q_k, \qquad\qquad (i,j)\in\hL;  \label{lossless Q}\\
	v_j^\mathrm{lin}(p, q) \!\!  & := &\!\!   v_0 + 2 \!\!\! \sum_{(k,l)\in\hP_j} \!\!\! 
		(r_{kl}P_{lk}^\mathrm{lin}+x_{kl}Q_{lk}^\mathrm{lin}),\\%  ~  j\in N^+.
	&&\qquad \qquad\qquad\quad  j=1,\ldots,n.
	\label{lossless v}
	\end{eqnarray*}
Given power injections  $(p,q)$,  $P_{ji}^\mathrm{lin}$ and $Q_{ji}^\mathrm{lin}$ 
are the aggregated real and reactive power injections downstream from
bus $j$ (in the subtree rooted at $j$).
If $P_{ji}^\mathrm{lin}>0$ (or $Q_{ji}^\mathrm{lin}>0$), there is more generation than load in 
the subtree rooted at $j$.  
This will likely, but not necessarily, produce reverse power flow, i.e., 
the actual power flows $(P_{ji}, Q_{ji})$ on line $(i,j)$ is likely to be upstream ($>0$), but may still be downstream ($<0$).
Note that $P^\mathrm{lin}$ is a linear function of $p$, $Q^\mathrm{lin}$ is a linear function 
of $q$, and $v^\mathrm{lin}$ is an affine function of $(p, q)$. 

Define $a^1_0:=1=:a^4_0$, $a^2_0:= 0 =: a^3_0$, and
	\begin{eqnarray*}
	a^1_i &:=& \prod_{(k,l)\in\hP_i} \left(1-\frac{2r_{kl} \left[ P_{lk}^\mathrm{lin}(\overline{p}) \right]^+}
				{\underline{v}_l}\right),\\
	a^2_i &:=& \sum_{(k,l)\in\hP_i} \frac{2r_{kl} \left[ Q_{lk}^\mathrm{lin}(\overline{q}) \right]^+}
				{\underline{v}_l},\\
	a^3_i &:=& \sum_{(k,l)\in\hP_i} \frac{2x_{kl} \left[ P_{lk}^\mathrm{lin}(\overline{p}) \right]^+}
				{\underline{v}_l},\\
	a^4_i &:=& \prod_{(k,l)\in\hP_i} \left(1-\frac{2x_{kl} \left[ Q_{lk}^\mathrm{lin}(\overline{q}) \right]^+}
				{\underline{v}_l}\right)
	\end{eqnarray*}
for $i\in N^+$. Define condition
\begin{itemize}
\item[\bf C1:] $a^1_i r_{ij} > a^2_i x_{ij}, ~a^3_i r_{ij} < a^4_i x_{ij}, ~(i,j)\in E$.
\end{itemize}
Condition C1 depends only on the network parameters $\overline{p}$, $\overline{q}$, $\underline{v}$ and 
the impedance $(r, x)$, and not on the power flow solutions.
Therefore it can be checked without first solving OPF or its relaxations.
 
Let $w^\mathrm{opt}=(p^\mathrm{opt},q^\mathrm{opt},P^\mathrm{opt},Q^\mathrm{opt},\ell^\mathrm{opt},v^\mathrm{opt},p_0^\mathrm{opt},q_0^\mathrm{opt})$ denote a solution of SOCP.  
\begin{theorem}\label{thm: main}
Suppose C1 holds.  
\bee
\item If every solution $w^\mathrm{opt}$ of SOCP satisfies
\begin{itemize}
\item[\bf C2:] $v_i^\mathrm{lin}\left(p^\mathrm{opt}, q^\mathrm{opt}\right) \leq \overline{v}_i, \quad i=1,\ldots,n,$
\end{itemize}
%\label{eq:tighterbnd}
then SOCP is exact.

\item If SOCP is exact, then OPF and SOCP have the same unique solution. 
\eee
\end{theorem}

\begin{proof}
Part 1 is proved in Section \ref{sec: math}, and part 2 is proved as follows. It is not difficult to verify that OPF and SOCP have the same solution when SOCP is exact (and has at least one solution). To complete the proof of part 2, it suffices to show that SOCP has a unique solution. Let $\tilde{w}=(\tilde{p},\tilde{q},\tilde{P},\tilde{Q},\tilde{\ell},\tilde{v},\tilde{p}_0,\tilde{q}_0)$ and $\hat{w}=(\hat{p},\hat{q},\hat{P},\hat{Q},\hat{\ell},\hat{v},\hat{p}_0,\hat{q}_0)$ denote two arbitrary solutions to SOCP, and define
	\begin{equation*}
	L^\mathrm{opt}:=L(\tilde{\ell}) = L(\hat{\ell})
	\end{equation*}
as the optimal value of SOCP. If SOCP is exact, then
	\begin{equation*}\label{eq: exact}
	\tilde{\ell}_{ij}\tilde{v}_j=\tilde{P}_{ji}^2+\tilde{Q}_{ji}^2, \quad \hat{\ell}_{ij}\hat{v}_j=\hat{P}_{ji}^2+\hat{Q}_{ji}^2
	\end{equation*}
for $(i,j)\in\hL$. For any $\theta\in(0,1)$, define
	\begin{equation*}
	w(\theta):=\theta \tilde{w}+(1-\theta)\hat{w}.
	\end{equation*}
The point $w(\theta)$ is feasible for SOCP since SOCP is convex. It is also optimal for SOCP because
	$$L(\ell(\theta)) = \theta L(\tilde{\ell}) + (1-\theta) L(\hat{\ell})=L^\mathrm{opt}.$$
If SOCP is exact, then
	\begin{eqnarray*}
	\ell_{ij}(\theta)v_j(\theta)=P_{ji}^2(\theta)+Q_{ji}^2(\theta)\label{eq: theta}
	\end{eqnarray*}
for $(i,j)\in\hL$. Substitute
	\begin{eqnarray*}
	& \ell_{ij}(\theta) = \theta \tilde{\ell}_{ij} + (1-\theta) \hat{\ell}_{ij}, ~v_j(\theta) = \theta \tilde{v}_j + (1-\theta) \hat{v}_j, &\\
	& P_{ji}(\theta) = \theta \tilde{P}_{ji} + (1-\theta) \hat{P}_{ji}, ~Q_{ji}(\theta) = \theta \tilde{Q}_{ji} + (1-\theta) \hat{Q}_{ji}&
	\end{eqnarray*}
in and simplify to obtain %using \eqref{eq: exact} to obtain
	\begin{equation*}
	\tilde{v}_j\hat{\ell}_{ij} + \hat{v}_j\tilde{\ell}_{ij} = 2\left(\tilde{P}_{ji}\hat{P}_{ji}+\tilde{Q}_{ji}\hat{Q}_{ji}\right)
	\end{equation*}
for $(i,j)\in\hL$. It follows that
	\begin{eqnarray*}
	&& 2\left(\tilde{P}_{ji}\hat{P}_{ji}+\tilde{Q}_{ji}\hat{Q}_{ji}\right)\\
	&=& \tilde{v}_j\frac{\hat{P}_{ji}^2+\hat{Q}_{ji}^2}{\hat{v}_j} + \hat{v}_j\frac{\tilde{P}_{ji}^2+\tilde{Q}_{ji}^2}{\tilde{v}_j}\\
	&=& \tilde{v}_j\frac{\hat{P}_{ji}^2}{\hat{v}_j} + \hat{v}_j\frac{\tilde{P}_{ji}^2}{\tilde{v}_j} + \tilde{v}_j\frac{\hat{Q}_{ji}^2}{\hat{v}_j} + \hat{v}_j\frac{\tilde{Q}_{ji}^2}{\tilde{v}_j}\\
	&\geq& 2\sqrt{\hat{P}_{ji}^2\tilde{P}_{ji}^2} + 2\sqrt{\hat{Q}_{ji}^2\tilde{Q}_{ji}^2}\\
	&\geq& 2\hat{P}_{ji}\tilde{P}_{ji} + 2\hat{Q}_{ji}\tilde{Q}_{ji}
	\end{eqnarray*}
for $(i,j)\in\hL$. The two inequalities must both attain equalities. The first inequality attaining equality implies that
	$$\frac{|\hat{P}_{ji}|}{\hat{v}_j}=\frac{|\tilde{P}_{ji}|}{\tilde{v}_j}, \quad \frac{|\hat{Q}_{ji}|}{\hat{v}_j}=\frac{|\tilde{Q}_{ji}|}{\tilde{v}_j}, \qquad (i,j)\in\hL.$$
The second inequality attaining equality implies that $\tilde{P}_{ji}\hat{P}_{ji}\geq0$, $\tilde{Q}_{ji}\hat{Q}_{ji}\geq0$ for $(i,j)\in\hL$. It follows that
	$$\frac{\hat{P}_{ji}}{\hat{v}_j}=\frac{\tilde{P}_{ji}}{\tilde{v}_j}, \quad \frac{\hat{Q}_{ji}}{\hat{v}_j}=\frac{\tilde{Q}_{ji}}{\tilde{v}_j}, \qquad (i,j)\in\hL.$$
Define $\eta_i:=\hat{v}_i/\tilde{v}_i$ for $i\in\hN$, then
	$$\hat{P}_{ji}=\eta_j\tilde{P}_{ji}, ~\hat{Q}_{ji}=\eta_j\tilde{Q}_{ji}, ~\hat{\ell}_{ij}=\eta_j\tilde{\ell}_{ij}, \quad (i,j)\in\hL.$$
Since $\eta_0=1$ and
	\begin{eqnarray*}
	\eta_i = \frac{\hat{v}_i}{\tilde{v}_i}= \frac{\hat{v}_j-2(r_{ij}\hat{P}_{ji}+x_{ij}\hat{Q}_{ji})+(r_{ij}^2+x_{ij}^2)\hat{\ell}_{ij}}
	{\tilde{v}_j-2(r_{ij}\tilde{P}_{ji}+x_{ij}\tilde{Q}_{ji})+(r_{ij}^2+x_{ij}^2)\tilde{\ell}_{ij}}=\eta_j
	\end{eqnarray*}
for $(i,j)\in\hL$, $\eta_i=1$ for $i\in\hN$. It implies $\tilde{P}=\hat{P}$, $\tilde{Q}=\hat{Q}$, $\tilde{\ell}=\hat{\ell}$, $\tilde{v}=\hat{v}$, and then $\tilde{p}=\hat{p}$, $\tilde{q}=\hat{q}$, $\tilde{p}_0=\hat{p}_0$, $\tilde{q}_0=\hat{q}_0$ follows. Therefore $\tilde{w}=\hat{w}$. Hence, SOCP has a unique solution.
\end{proof}

\begin{remark}\label{rem: generalization}
In part 1, the objective function $L(\ell)$ can be generalized to $f\left(L(\ell),p,q\right)$ where the function $f(x,y,z):\mathbb{R}\times\mathbb{R}^n\times\mathbb{R}^n\rightarrow\mathbb{R}$ is strictly increasing in $x$. It is important for the proof that $f$ depends on $L(\ell)$ instead of $\ell$ itself. The power injection constraints in \eqref{constraint s} can be generalized to $(p,q)\in\mathcal{X}$ where $\mathcal{X}$ is an arbitrary set. In particular, $\mathcal{X}$ can be nonconvex or discrete.

In part 2, the objective function $L(\ell)$ can be generalized to any convex function $f(w)$. The power injection constraints in \eqref{constraint s} can be generalized to $(p,q)\in\mathcal{X}$ where $\mathcal{X}$ is an arbitrary convex set.
\end{remark}




%Theorem \ref{thm: main}  implies that C1 guarantees exact relaxation if there are no upper bounds (i.e., they are nonbinding) on voltage magnitudes. We will return to C1 later in Section \ref{sec:C1} to show that they seem to hold in practice.   Meanwhile we explore a more important implication of Theorem \ref{thm: main}.
